Matching while Learning

We consider the problem faced by a service platform that needs to match limited supply with demand but also to learn the attributes of new users in order to match them better in the future. We introduce a benchmark model with heterogeneous "workers" (demand) and a limited supply of "jobs" that arrive over time. Job types are known to the platform, but worker types are unknown and must be learned by observing match outcomes. Workers depart after performing a certain number of jobs. The expected payoff from a match depends on the pair of types and the goal is to maximize the steady-state rate of accumulation of payoff. Though we use terminology inspired by labor markets, our framework applies more broadly to platforms where a limited supply of heterogeneous products is matched to users over time. Our main contribution is a complete characterization of the structure of the optimal policy in the limit that each worker performs many jobs. The platform faces a trade-off for each worker between myopically maximizing payoffs (exploitation) and learning the type of the worker (exploration). This creates a multitude of multi-armed bandit problems, one for each worker, coupled together by the constraint on availability of jobs of different types (capacity constraints). We find that the platform should estimate a shadow price for each job type, and use the payoffs adjusted by these prices, first, to determine its learning goals and then, for each worker, (i) to balance learning with payoffs during the "exploration phase," and (ii) to myopically match after it has achieved its learning goals during the "exploitation phase."

==> algobox-yk.tex <==
\\
\fbox{{\footnotesize\begin{minipage}{\textwidth}
\begin{center} {\normalsize \bf DEEM: Decentralized exploration-then-exploitation for matching} \end{center}
\textbf{Input parameters:} $\cI$, $\cJ$, $A$, $\rho$, $\mu$, N.\\
{\bf Compute:}\begin{itemize}
\item $\alpha(i) = \alpha(i,\cI, \cJ, A, \rho, \mu)$ for all $i$ (Optimal policy for confirming type $i$)
\item $y^* = y(\cI, \cJ, A, \rho, \mu, N)$ (Routing {\color{blue} matrix} during exploitation)
\end{itemize}

{\bf Initialization:}\begin{itemize}
\item $\lambda(i) \leftarrow \rho(i)$ for all $i\in \cI$ (the un-normalized posterior probabilities; initialized to the prior)
\item $\MAP \leftarrow \argmax_{i\in\cI} \lambda(i)$ (initialization of the MAP estimate)
\item $Label \leftarrow \phi$ (worker label; initially unassigned, denoted by $\phi$)
\end{itemize}
{\bf For $k = 0,\ldots, N-1$:}
\begin{itemize}
\item[]{\bf If} $Label = \phi$:
	\begin{itemize}
	\item Assign job type $j^*_k$ =  Explore(N, $\lambda$, \MAP, $\alpha$)
	\item Obtain observation $X_k$
	\item $\lambda(i) \leftarrow \lambda(i) \times (A(i,j)\mathbf{1}_{\{X_k=1\}}+(1-A(i,j))\mathbf{1}_{\{X_k=0\}})$
	%\item $\MAP \leftarrow \argmax_{i\in\cI} \lambda(i)$
	\item {\bf If} $\min_{i\neq MAP}\frac{\lambda(MAP)}{\lambda(i)} \geq \log N$ and $\min_{i'\in \Str(MAP)}\frac{\lambda(MAP)}{\lambda(i)} \geq N$: (Transition to Exploitation)
		\begin{itemize}
		\item[] $Label \leftarrow MAP$  (Worker label assigned)
		\end{itemize}
	
	\end{itemize}
\item[] {\bf Else}:
	\begin{itemize}
		\item Assign job type $j^*_k$= Exploit($Label$, $y^*$)
	\end{itemize}
\end{itemize}
\end{minipage}}}

\fbox{{\footnotesize\begin{minipage}{\textwidth}
\begin{center} {\normalsize \bf Definitions} \end{center}
Def Explore(N, $\lambda$, \MAP, $\alpha$) :
\begin{itemize}
\item[] {\bf If} $\min_{i\neq \MAP}\frac{\lambda(\MAP)}{\lambda(i)} <\log N$: (Guessing)
		\begin{itemize}
		\item[] $j^* \sim Uniform(\cJ)$
		\end{itemize}
\item[] {\bf Else}: (Confirmation)
		\begin{itemize}
		\item[] $j^* \sim \alpha(\MAP)$
		\end{itemize}
\item[] {\bf Return} $j^*$
\end{itemize}


Def Exploit($Label$, $y^*$) :
\begin{itemize}
	\item[] $j^* \sim y^*(Label, .)$
	\item[] {\bf Return} $j^*$
\end{itemize}

Def $\alpha(i,\cI, \cJ, A, \rho, \mu):$
\begin{itemize}
\item {\bf Shadow Prices.} Define $p^*$ as the vector of optimal shadow prices for the capacity constraint \eqref{eq:opt2} in the problem with known types \eqref{eq:opt1}--\eqref{eq:opt3}. Under the generalized imbalance condition \eqref{eqn:genimb}, we show that these prices are uniquely determined; see Proposition \ref{prop:uniqueness_of_prices} in Appendix~\ref{apx:otherproofs}.
\item {\bf $\Str(i)$: Strong distinction goals for confirming type $i$.} Define $\Str(i) = \{ i' : \cS(i) \setminus \cS(i') \neq \emptyset \}$, where \ecl\cS(i)=\arg\max_{j\in \cS} A(i,j)-p^*(j)\ecr is the set of optimal job types for worker type $i$.
\item Let \ecl U(i) = \max_{j \in \cS} A(i,j) - p^*(j) \ecr denote the maximal externality-adjusted payoff of worker type $i$. Define the set,
\begin{align}\label{eqn:alpha}
\mathcal{A}(i) &= \argmin_{\alpha\in \Delta(\cS)}\frac{\sum_{j\in \cS} \alpha_j\big(U(i)-[A(i,j)-p^*(j)]\big)}{\min_{i'\in \Str(i)}\sum_{j\in \cS}\alpha_j\KL(i,i'|j)},
\end{align}
where $\KL(i,i'|j)$ is the Kullback--Leibler divergence\footnote{The KL divergence between a Bernoulli($q$) and a Bernoulli($q'$) distribution is defined as $q\log{\frac{q}{q'}} +(1-q) \log{\frac{1-q}{1-q'}}$.} between the distributions $\Bern(A(i,j))$ and $\Bern(A(i',j))$, and $\Delta(\cS)$ is the set of distributions over $\cS$. Then return $\alpha(i)$ such that
\begin{equation}
\alpha(i) \in \argmax_{\alpha\in\mathcal{A}(i)}\min_{i'\in \Str(i)}\sum_{j\in \cS}\alpha_j\KL(i,i'|j),
\end{equation}
breaking ties arbitrarily.  In Appendix~\ref{apx:alpha}, we show that \eqref{eqn:alpha} can be written as a small linear program.
\end{itemize}
Def $y^* = y(\cI, \cJ, A, \rho, \mu, N):$ Uses Explore()
\end{minipage}}} 
